The Science Case for LIGO-India

The global network of gravitational-wave detectors has completed three observing runs with $\sim 50$ detections of merging compact binaries. A third LIGO detector, with comparable astrophysical reach, is to be built in India (LIGO-Aundha) and expected to be operational during the latter part of this decade. Multiple detectors operating at different parts of the globe will provide several pairs of interferometers with longer baselines and an increased network SNR. This will improve the sky localisation of GW events. Multiple detectors simultaneously in operation will also increase the baseline duty factor, thereby, leading to an improvement in the detection rates and, hence, the completeness of surveys. In this paper, we quantify the improvements due to the expansion of the LIGO Global Network (LGN) in the precision with which source properties will be measured. We also present examples of how this expansion will give a boost to tests of fundamental physics.

==> app1.tex <==
\begin{figure}
	\centering
	\includegraphics[width=\columnwidth]{dutycycle2.png}
	\caption{Effective duty cycle of various network configurations as a function of the individual duty cycle \Rana{Who's plot is this? replace w PDF}}
	\label{fig:dutycycle}
\end{figure}



==> matter.tex <==
\subsection{Matter effects of neutron star}
\label{sec:PE}
\cmt{Assigned to: Arunava, Sukanta?. This section should be moved to the EM-alert section.} 

\cmt{Timeline: PE-runs are just launched.} 

This subsection will be focused on how the source classification can be improved and the probability of presence of EM-bright signals with the presence of LIO-Aundth detector at A+ sensitivity. 



==> multimess.tex <==

\section{Multimessenger astronomy}
	\cmt{Assigned to: Saleem, Arun and Archana} 
	This is a joint implication of the increased  event rates and the improved inclination angle  estimation. Inclination angle is referred to as viewing angle $\tv$ in GRB literature. 
	The observed short GRB energetics is a consequence of the convolution of the intrinsic energetics and the observer's viewing angle $\tv$. For example, the bursts with very large $\tv$ are very unlikely to be detected. From the joint observation of GW and GRB, one can constrain $\tv$ better than from individual measurements.  
	
	There are different structured jet models proposed in literature. That includes a uniform top hat jet model where a the energy and Lorents factor of the ejected material is distributed over a uniform cone of some typical opening angle. This model explained many of the observed features of short and long bursts prior to the detection of GW170817 and assocuiated GRB170817A, whereas this model has not been able to explain the observed features of GRB170817A completely and therefore it's validity is still under debate. Alternative models include a Gaussian structured jet where the energy and Lorentz factor follows a Gaussian profile and further there is a power-law jet model. The chances of detecting the bursts for larger viewing angle will crucially depend on the jet structure. This implies to the fact that the observed viewing angle distributions will carry signatures of the jet structure. Or in other words, the  
	statistical distributions of $\tv$  of the joint GW-GRB detection events will change for each of these models. We ask a question how many events are required to distinguish between jet models based on the observed veiwing angle distributions. Miller et al 2015 (and saleem et al 2018- a work in progress) have quantified the minimum number of events required to make this distinctions. LIGO-India, as we discussed dbefore, will increase the number of joint detections, and hence will contribute towards this front (\tcr{more quantified statements to be added}).



==> stoch.tex <==
\section{Stochastic Background}
%	\cmt{Assigned to: Jishnu and Sudhagar}

In this section, we are comparing the performance of a network of baselines with that of its individual baselines for a directed search of a Stochastic gravitational wave background. 

Various techniques have been proposed and developed to search for isotropic and anisotropic SGWB in data from detectors in different bands. For ground-based multiple GW detectors, data from pairs of detectors are cross-correlated to look for a stochastic signal. Along with the cross-correlated searches for SGWB, the standard technique presently used in many of the analyses is the GW radiometer algorithm. The GW radiometer algorithm considers the delay in the GW signal arrival at detectors that are geographically separated. A raw sky-map produced by this analysis is referred to as the `dirty map'. A dirty map is a convolution of the true source map with the antenna response of the detectors along with some additive noise. The estimate of the true source distribution in the sky, the `clean map', can be obtained  by undoing these artefacts introduced by the detector's antenna pattern through a procedure called deconvolution.  In the case of SGWB map-making, the deconvolution process introduces a considerable amount of noise in the cleaned map because of insensitive modes of the beam. Usually, some form of regularisation is used to tackle these issues. On the other hand, when we consider a network of detectors, which are oriented differently, will have less number of insensitive modes.  Hence the network acts as a natural regulariser.

Following the radiometer algebra, one can frame the SGWB search in terms of a dirty map, the GW sky seen through the detector's response matrix. For a baseline $\mathcal{I}$, the dirty map can be written as,
\begin{equation}
X_p =  \sum_{Ift} \gamma^{I*}_{ft,p} \frac{ H(f)} {P_{\mathcal{I}_1}(t;f) P_{\mathcal{I}_2}(t;f)}  C^{I} (t;f)\,. 
\label{eq:SGWB_Dirty_map}
\end{equation}
%
Here $C^{I} (t;f)$ represents the cross correlation statistic(CSD) at a time $t$. 
The uncertainty in the above observed dirty map can be expressed in terms of the Fisher information matrix as,
\begin{equation}
\Gamma_{pp'} = \sum_{Ift} \frac{H^2(f)}{P_{\mathcal{I}_1}(t;f) \, P_{\mathcal{I}_2}(t;f)} \,\gamma^{I*}_{ft,p} \, \gamma^{I}_{ft,p'} \, .
\label{eq:SGWB_Fisher}
\end{equation}
The variable $\gamma$ in the above equations represents a detector dependent function known as the Overlap Reduction Function(ORF). It is given as, 
\begin{equation}
\gamma_{ft,p} ^{I} := \sum_{A} \int_{S^2} d \mathbf{\hat \Omega} F^{A}_{\mathcal{I}_1}(\mathbf{\hat \Omega},t) 
F^{A}_{\mathcal{I}_2}(\mathbf{\hat\Omega},t) e^{2\pi i f \frac{\mathbf{\hat \Omega}\cdot {\mathbf{\Delta x}_I (t)}}{c}} e_p(\mathbf{\hat \Omega}) \, .
\label{eq:SGWB_ORF}
\end{equation}
%
\begin{figure}
\centering
\includegraphics[width = 0.65 \linewidth]{SGWB_HLA_orf.pdf}
\caption{The overlap reduction function calculated for all the three baselines.}
\label{fig:orf_stochastic}		
\end{figure}
%
$F^{A}_{\mathcal{I}}(\mathbf{\hat \Omega},t)$ denotes the antenna pattern function, which record the response of the detector pair, constituting a baseline $\mathbf{\Delta x}_I (t)$, to a GW with polarization $A= +,\times$.  The ORF calculated for the three baselines of interest are shown in~Fig.\ref{fig:orf_stochastic}.

In this analysis, we will compute and study the ill-posedness of the Fisher matrix given in Eq.\ref{eq:SGWB_Fisher} for all the three baselines. We have simulated the folded data set for all the three baseline assuming their design sensitivity by following the steps described in~\cite{Ain_Folding}. The simulated dataset consists of $898$~frames of CSDs and PSDs. Each with a $50$\% overlapping segment duration of $192$~sec which spans one sidereal day. We then run radiometer search using the {\tt{PyStoch}} pipeline~\cite{pystoch_2018} in the spherical harmonic basis~\cite{sph_pystoch_2020} for a frequency range from 20-500Hz and with a power-law spectral indices $\alpha=3$ and have $l_{\rm{max}} = 30$. We then calculate the eigenvalues of the estimated Fisher matrix for HL, AH, AL baselines along with the combined AHL network.  
%
\begin{figure}
\centering
\includegraphics[width = 0.65 \linewidth]{SGWB_fisher_eigenvalues.pdf}
\caption{Eigenvalues of the Fisher information matrix $\Gamma_{lm,l'm'}$ is represented using the solid line. The dotted vertical line demarcates the eigenvalues considered for the inversion of regularized Fisher matrix to obtain the clean map. For demonstration, we have considered $l_{\rm{max}}=30$ (961 modes).}
\label{fig:eigenvalue_fisher}		
\end{figure}
%
We have analysed these eigenvalues and check how the condition the number of the Fisher matrix improves by the introduction of LIGO-Aundha detector. In~Fig.\ref{fig:eigenvalue_fisher}, we show the above obtained eigenvalues for all the possible cases. The dotted vertical line demarcates the eigenvalues that were considered in the LVK stochastic analysis (to regularize the matrix). It's evident form this figure that, the number of modes that can be considered for defining an upper-limit, computing the $C_l$, etc significantly increases as we introduce the third LIGO detector.

